Collapsible Pushdown Parity Games

This paper studies a large class of two-player perfect-information turn-based parity games on infinite graphs, namely those generated by collapsible pushdown automata. The main motivation for studying these games comes from the connections from collapsible pushdown automata and higher-order recursion schemes, both models being equi-expressive for generating infinite trees. Our main result is to establish the decidability of such games and to provide an effective representation of the winning region as well as of a winning strategy. Thus, the results obtained here provide all necessary tools for an in-depth study of logical properties of trees generated by collapsible pushdown automata/recursion schemes.

==> Notations.tex <==
\begin{center}
{\LARGE Notations}	
\end{center}

\begin{itemize}
	\item Arena: $\arena$
	\item Game: $\game=(\arena,\WC)$. The initial vertex is not part of the game 
	\item Colours / colouring function: $\colors$ / $\col$
	\item stack: $\stack$; if needed $\varstack$
\end{itemize}

\newpage
